NICER/NuSTAR Characterization of 4U 1957+11: A Near Maximally Spinning Black Hole Potentially in the Mass Gap

4U 1957+11 is a black hole candidate system that has been in a soft X-ray spectral state since its discovery. We present analyses of recent joint NICER and NuSTAR spectra, which are extremely well-described by a highly inclined disk accreting into a near maximally spinning black hole. Owing to the broad X-ray coverage of NuSTAR the fitted spin and inclination are strongly constrained for our hypothesized disk models. The faintest spectra are observed out to 20 keV, even though their hard tail components are almost absent when described with a simple corona. The hard tail increases with luminosity, but shows clear two track behavior with one track having appreciably stronger tails. The disk spectrum color-correction factor is anti-correlated with the strength of the hard tail (e.g., as measured by the Compton $y$ parameter). Although the spin and inclination parameters are strongly constrained for our chosen model, the mass and distance are degenerate parameters. We use our spectral fits, along with a theoretical prior on color-correction, an observational prior on likely fractional Eddington luminosity, and an observational prior on distance obtained from Gaia studies, to present mass and distance contours for this system. The most likely parameters, given our presumed disk model, suggest a 4.6 $\mathrm{M_\odot}$ black hole at 7.8 kpc observed at luminosities ranging from $\approx 1.7\%$--$9\%$ of Eddington. This would place 4U 1957+11 as one of the few actively accreting sources within the `mass gap' of ${\approx} 2$--$5\,\mathrm{M_\odot}$ where there are few known massive neutron stars or low mass black holes. Higher mass and distance, however, remain viable.

==> table_polykerr_calibration.tex <==
\begin{deluxetable*}{rcccccc} 
\setlength{\tabcolsep}{0.05in} 
\tabletypesize{\footnotesize} 
\tablewidth{0pt} 
\tablecaption{``Calibration'' parameters for Comptonized disk fits to joint \nicer/\nustar spectra.} 
\tablehead{ 
 Epoch 
   & \colhead{$E_{e}$} & \colhead{$\tau_{e}$} 
   & \colhead{$E_{a1}$} & \colhead{$S_{a1}$} 
   & \colhead{$E_{a2}$} & \colhead{$S_{a2}$} \\ 
   & \colhead{(keV)} & 
   & \colhead{(keV)} & \colhead{($\times10^{-3}$)} 
   & \colhead{(keV)} & \colhead{($\times10^{-3}$)} } 
\startdata 
   2  
 & \errtwo{0.98}{0.03}{0.03} 
 & \errtwo{0.08}{0.02}{0.01} 
 & \errtwo{0.568}{0.005}{0.005} 
 & \errtwo{21.9}{4.3}{3.6} 
 & \errtwo{0.758}{0.023}{0.007} 
 & \errtwo{1.7}{2.0}{1.5} 
   \\   4  
 & \errtwo{1.00}{0.01}{0.01} 
 & \errtwo{0.07}{0.01}{0.01} 
 & \errtwo{0.572}{0.003}{0.003} 
 & \errtwo{23.7}{2.5}{2.3} 
 & \errtwo{0.768}{0.007}{0.006} 
 & \errtwo{5.9}{1.0}{0.8} 
   \\   6  
 & \errtwo{0.98}{0.01}{0.01} 
 & \errtwo{0.05}{0.00}{0.01} 
 & \errtwo{0.573}{0.002}{0.003} 
 & \errtwo{22.8}{2.2}{2.2} 
 & \errtwo{0.763}{0.006}{0.005} 
 & \errtwo{6.0}{0.7}{0.7} 
   \\   7  
 & \errtwo{1.00}{0.00}{0.01} 
 & \errtwo{0.07}{0.00}{0.01} 
 & \errtwo{0.572}{0.003}{0.002} 
 & \errtwo{22.3}{2.1}{2.0} 
 & \errtwo{0.763}{0.006}{0.006} 
 & \errtwo{4.3}{0.6}{0.6} 
   \\   8  
 & \errtwo{0.99}{0.01}{0.01} 
 & \errtwo{0.07}{0.00}{0.01} 
 & \errtwo{0.571}{0.003}{0.003} 
 & \errtwo{21.6}{2.2}{1.9} 
 & \errtwo{0.759}{0.006}{0.004} 
 & \errtwo{4.9}{0.7}{0.6} 
   \\   9  
 & \errtwo{0.97}{0.01}{0.01} 
 & \errtwo{0.06}{0.00}{0.01} 
 & \errtwo{0.572}{0.002}{0.002} 
 & \errtwo{24.4}{2.4}{2.1} 
 & \errtwo{0.758}{0.005}{0.004} 
 & \errtwo{7.2}{0.7}{0.8} 
   \\   10  
 & \errtwo{0.98}{0.01}{0.01} 
 & \errtwo{0.07}{0.01}{0.01} 
 & \errtwo{0.571}{0.004}{0.003} 
 & \errtwo{21.1}{2.4}{2.4} 
 & \errtwo{0.763}{0.007}{0.008} 
 & \errtwo{4.9}{1.0}{0.9} 
   \\\enddata 
\tablecomments{\tcompkerrcal} 
\end{deluxetable*} 

